On Semi-Supervised Estimation of Distributions

We study the problem of estimating the joint probability mass function (pmf) over two random variables. In particular, the estimation is based on the observation of $m$ samples containing both variables and $n$ samples missing one fixed variable. We adopt the minimax framework with $l^p_p$ loss functions, and we show that the composition of uni-variate minimax estimators achieves minimax risk with the optimal first-order constant for $p \ge 2$, in the regime $m = o(n)$.

==> macros/course_header.tex <==
%\pagestyle{myheadings}
%\markright{P. Golland and G. W. Wornell}
\newcommand{\thecoursename}{
Massachusetts Institute of Technology \\
Department of Electrical Engineering and Computer Science

\textsc{6.437 Inference and Information}
}

\newcommand{\theterm}{Spring 2016}
\thispagestyle{empty}



==> macros/defs.tex <==
\newcommand{\courseheader}{
\vspace*{-1in}
\begin{center}
\thecoursename \\
\theterm
\vspace*{0.1in}
\hrule
\end{center}
}

\newcounter{psctr}
\newcounter{probctr}[psctr]
%\renewcommand{\theprobctr}{\arabic{psctr}.\arabic{probctr}}
\newcommand{\problem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr}\nopagebreak

\noindent{#1}

}
\newcommand{\extraproblem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr\ (practice)}\nopagebreak

\noindent{#1}

}

\newcommand{\putfig}[3]{%
\centering
\includegraphics[width=#2]{#1}
\caption{#3}
}

\newcommand{\putfigtwo}[4]{%
\centering
\subfloat[\ ]{\includegraphics[width=#3]{#1}}\\ \vspace*{3ex}
\subfloat[\ ]{\includegraphics[width=#3]{#2}}
\caption{#4}
}

\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\DeclareMathAlphabet{\mathbbb}{U}{bbold}{m}{n}  % bb bold numbers
% can also use bbm package, which seems to work w/o pdflatex

%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbb}{bbold}


% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}  
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

\newcommand{\fxfm}{\stackrel{\mathcal{F}}{\longleftrightarrow}}
\newcommand{\lxfm}{\stackrel{\mathcal{L}}{\longleftrightarrow}}
\newcommand{\zxfm}{\stackrel{\mathcal{Z}}{\longleftrightarrow}}

\DeclareMathOperator*{\gltop}{\gtreqless}
\newcommand{\glt}{\;\gltop^{\Hh=\svH_1}_{\Hh=\svH_0}\;}
\newcommand{\glty}{\;\gltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\gltby}{\;\gltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\DeclareMathOperator*{\geltop}{\genfrac{}{}{0pt}{}{\ge}{<}}
\newcommand{\gelty}{\;\geltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\geltby}{\;\geltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
%\renewcommand{\pe}{\Prob{e}}
\renewcommand{\defeq}{\triangleq}
\newcommand{\like}{\svlike}
\newcommand{\rvlike}{\mathssf{L}}
\newcommand{\sst}{\cl}
\newcommand{\svlike}{L}
\newcommand{\llike}{\rvllike}
\newcommand{\rvllike}{\cl}
\newcommand{\svllike}{l}
\newcommand{\lliket}{\tel}
\newcommand{\bllike}{\rvbllike}
\newcommand{\rvbllike}{\boldsymbol{\cl}}
\newcommand{\svbllike}{\mathbf{l}}
\newcommand{\Qb}{\overline{Q}}
\renewcommand{\comb}[2]{\binom{#1}{#2}}


%% Random/sample variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
% Capitals
\newcommand{\rvA}{{\mathssf{A}}}	% A
\newcommand{\svA}{A}
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\svbA}{{\mathbf{A}}}
\newcommand{\rvFh}{{\hat{\mathssf{F}}}}	% F
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvHh}{{\hat{\mathssf{H}}}}	% H
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\svH}{H}
\newcommand{\svHh}{{\hat{\svH}}}
\newcommand{\rvL}{{\mathssf{L}}}	% L
\newcommand{\svL}{L}
\newcommand{\rvN}{{\mathssf{N}}}	% N
\newcommand{\rvR}{{\mathssf{R}}}	% R
\newcommand{\rvRh}{{\hat{\rvR}}}
\newcommand{\rvS}{{\mathssf{S}}}	% S
\newcommand{\rvSh}{{\hat{\rvS}}}
\newcommand{\rvW}{{\mathssf{W}}}	% W
\newcommand{\rvX}{{\mathssf{X}}}  	% X, random variable
\newcommand{\svX}{X}		  	
\newcommand{\rvXt}{{\tilde{\rvX}}}
\newcommand{\rvY}{{\mathssf{Y}}}	% Y

\newcommand{\rvZ}{{\mathssf{Z}}}	% Z
\newcommand{\rvbZ}{{\mathbsf{Z}}}	
\newcommand{\svZ}{{{Z}}}	
\newcommand{\svbZ}{{\mathbf{Z}}}	

\newcommand{\rva}{{\mathssf{a}}}	% a
\newcommand{\rvah}{{\hat{\rva}}}
\newcommand{\sva}{a}
\newcommand{\svah}{{\hat{\sva}}}
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\svba}{{\mathbf{a}}}
%
\newcommand{\rvb}{{\mathssf{b}}}	% b
\newcommand{\rvbh}{{\hat{\rvb}}}
\newcommand{\svb}{b}
\newcommand{\svbh}{{\hat{\svb}}}
\newcommand{\rvbb}{{\mathbsf{b}}}
\newcommand{\svbb}{{\mathbf{b}}}
%
\newcommand{\rvc}{{\mathssf{c}}}	% c
\newcommand{\rvch}{{\hat{\rvc}}}
\newcommand{\svc}{c}
\newcommand{\svch}{{\hat{\svc}}}
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\svbc}{{\mathbf{c}}}
%
\newcommand{\rvbd}{{\mathbsf{d}}}	% d
\newcommand{\rve}{{\mathssf{e}}}	% e
\newcommand{\sve}{e}
\newcommand{\rvbfe}{{\mathbsf{e}}}
\newcommand{\svbfe}{{\mathbf{e}}}
\newcommand{\rvf}{{\mathssf{f}}}	% f
\newcommand{\svf}{f}
\newcommand{\rvbff}{{\mathbsf{f}}}
\newcommand{\svbff}{{\mathbf{f}}}
\newcommand{\rvg}{{\mathssf{g}}}	% h
\newcommand{\svg}{g}
\newcommand{\rvh}{{\mathssf{h}}}	% h
\newcommand{\rvk}{{\mathssf{k}}}	% k
\newcommand{\svk}{k}
\newcommand{\rvm}{{\mathssf{m}}}	% m
\newcommand{\rvbm}{{\mathbsf{m}}}  
\newcommand{\svm}{{{m}}}
\newcommand{\svbm}{{\mathbf{m}}}
\newcommand{\rvn}{{\mathssf{n}}}	% n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvq}{{\mathssf{q}}}	% q
\newcommand{\svq}{q}
\newcommand{\rvr}{{\mathssf{r}}}	% r
\newcommand{\rvbr}{{\mathbsf{r}}}
\newcommand{\svr}{{r}}
\newcommand{\svbr}{{\mathbf{r}}}
\newcommand{\rvs}{{\mathssf{s}}}	% s
\newcommand{\svs}{s}
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\svbs}{{\mathbf{s}}}
\newcommand{\rvt}{{\mathssf{t}}}	% t
\newcommand{\svt}{t}
\newcommand{\rvbt}{{\mathbsf{t}}}
\newcommand{\svbt}{{\mathbf{t}}}
\newcommand{\rvu}{{\mathssf{u}}}	% u
\newcommand{\svu}{u}
\newcommand{\svuh}{{\hat{\svu}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvv}{{\mathssf{v}}}	% v
\newcommand{\svv}{v}
\newcommand{\svvh}{{\hat{\svv}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvvh}{{\hat{\rvv}}}
\newcommand{\rvw}{{\mathssf{w}}}	% w
\newcommand{\svw}{w}
\newcommand{\rvwh}{{\hat{\rvw}}}
\newcommand{\svwh}{{\hat{\svw}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvx}{{\mathssf{x}}}	% x, random variable
\newcommand{\rvxh}{{\hat{\rvx}}}
\newcommand{\rvxt}{{\tilde{\rvx}}}
\newcommand{\svx}{x}			% sample value
\newcommand{\svxh}{{\hat{\svx}}}
\newcommand{\svxt}{{\tilde{\svx}}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvbxh}{{\hat{\rvbx}}}
\newcommand{\rvbxt}{{\tilde{\rvbx}}}
\newcommand{\svbx}{{\mathbf{\svx}}}
\newcommand{\svbxt}{{\tilde{\svbx}}}
\newcommand{\svbxh}{{\hat{\mathbf{x}}}}
\newcommand{\rvy}{{\mathssf{y}}}	% y
\newcommand{\rvyh}{{\hat{\mathssf{y}}}}
\newcommand{\svy}{y}
\newcommand{\rvyt}{{\tilde{\rvy}}}
\newcommand{\svyt}{{\tilde{\svy}}}
\newcommand{\svyh}{{\hat{\svy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvbyt}{{\tilde{\rvby}}}
\newcommand{\svby}{{\mathbf{y}}}
\newcommand{\svbyt}{{\tilde{\svby}}}
\newcommand{\rvz}{{\mathssf{z}}}	% z
\newcommand{\rvzh}{{\hat{\rvz}}}
\newcommand{\rvzt}{{\tilde{\rvz}}}
\newcommand{\svz}{z}
\newcommand{\svzh}{{\hat{\svz}}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svbz}{{\mathbf{z}}}

% Handle uppercase Greek differently
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

\newcommand{\ddx}{\frac{\diff}{\diff \svx}}
\newcommand{\ddbx}{\frac{\diff}{\diff\svbx}}
\newcommand{\ppx}{\frac{\p}{\p \svx}}
\newcommand{\ppbx}{\frac{\p}{\p\svbx}}
\newcommand{\ddy}{\frac{\diff}{\diff \svy}}
\newcommand{\ddby}{\frac{\diff}{\diff\svby}}
\newcommand{\ppy}{\frac{\p}{\p \svy}}
\newcommand{\ppby}{\frac{\p}{\p\svby}}

\def\setTh{\text{$\mksetTh$}}  % make caligraphic Theta
\def\mksetTh{\setbox0\hbox{$\mathcal{O}$}%
    \rlap{\hbox to \wd0{\hss\raisebox{.2ex}{\hspace*{.07em}\textbf{-}}\hss}}\box0}

%  --add new macros below this line--

\newcommand\indep{\protect\mathpalette{\protect\indepT}{\perp}}
\def\indepT#1#2{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}
\newcommand{\truex}{\svx}
\newcommand{\obsy}{\svy}
\newcommand{\dummyx}{a}
\newcommand{\dummybx}{\ba}
\newcommand{\dummyy}{b}
\newcommand{\dummyby}{\bb}
\newcommand{\dummyz}{c}
\newcommand{\Db}{D_\mathrm{B}}   % binary divergence
\newcommand{\Hb}{H_\mathrm{B}}   % binary entropy
\newcommand{\Hhb}{\Hh_\mathrm{B}} % Bayes decision rule
\newcommand{\Hhnp}{\Hh_\mathrm{NP}} % Neyman-Pearson decision rule
\newcommand{\Hhm}{\Hh_\mathrm{M}} % minimax decision rule
\newcommand{\alphA}{\cA}
\newcommand{\alphB}{\cB}
\newcommand{\alphE}{\cE}
\newcommand{\alphL}{\cL}
\newcommand{\alphV}{\cV}
\newcommand{\cardV}{M}
\newcommand{\alphR}{\cR}
\newcommand{\alphS}{\cS}
\newcommand{\alphT}{\cT}
\newcommand{\alphU}{\cU}
\newcommand{\alphW}{\cW}
\newcommand{\alphX}{\cX}
\newcommand{\cardX}{L}
\newcommand{\alphY}{\cY}
\newcommand{\alphZ}{\cZ}
\newcommand{\cardY}{M}
\newcommand{\efdim}{K}
\newcommand{\dimX}{K}
\newcommand{\dimY}{N}
\newcommand{\alphH}{\cH}

\newcommand{\sumX}{\sum_{\svx\in\alphX}}
\newcommand{\sumY}{\sum_{\svy\in\alphY}}

\newcommand{\fisher}{J}
\newcommand{\Fisher}{\bJ}
\newcommand{\bfisher}{\bJ}
\newcommand{\score}{S}
\newcommand{\Score}{\bS}
\newcommand{\bscore}{\bS}
\newcommand{\objfn}{\varphi}
\newcommand{\varobjfn}{\tilde{\objfn}}




\renewcommand{\emptyset}{\varnothing}
\renewcommand{\approx}{\cong}

% functional dot

\def\fndot{\, \cdot \,}

% exponential

\newcommand{\eexp}[1]{e^{#1}}

% iid

\newcommand{\iid}{i.i.d.}

% convergence

\newcommand{\convp}{\stackrel{\mathrm{p}}{\longrightarrow}}
\newcommand{\convas}{\stackrel{\mathrm{a.s.}}{\longrightarrow}}
\newcommand{\convwpone}{\convas}
\newcommand{\convd}{\stackrel{\mathrm{d}}{\longrightarrow}}
\newcommand{\convD}{\stackrel{\mathrm{D}}{\longrightarrow}}

% stochastic approximation

\newcommand{\pun}{p_\circ}
\newcommand{\punh}{\hat{p}_\circ}
\newcommand{\qun}{q_\circ}
\newcommand{\qunh}{\hat{q}_\circ}

\newcommand{\genf}{f}
\newcommand{\genfb}{\bar{f}}
\newcommand{\genfbh}{\hat{\bar{\rvf}}}


\DeclareMathOperator{\neb}{ne}
\newcommand{\bep}{{\boldsymbol{\varepsilon}}}

\newcommand{\gauss}{\mathtt{N}}
\newcommand{\bern}{\mathtt{B}}
\newcommand{\unif}{\mathtt{U}}
\newcommand{\poiss}{\mathtt{P}}
\newcommand{\betad}{\mathtt{Beta}}
\newcommand{\gammad}{\mathtt{Gamma}}
\newcommand{\expd}{\mathtt{E}}
\newcommand{\expfam}{\mathcal{E}}

\newcommand{\kron}{\mathbbb{1}}
%\newcommand{\kron}{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
%\DeclareMathOperator{\kron}{\leavevmode\hbox{\small\rm1\normalsize\kern-.33em1}}

\newcommand{\dotleq}{\stackrel{.}{\leq}}
\newcommand{\dotlt}{\stackrel{.}{<}}
\newcommand{\dotgeq}{\stackrel{.}{\geq}}
\newcommand{\dotgt}{\stackrel{.}{>}}
\newcommand{\Ps}[1]{P\left\{#1\right\}}
\newcommand{\Qs}[1]{Q\left\{#1\right\}}

\newcommand{\diff}{\mathrm{d}}

% from 6.008

\newcommand{\sd}{p_\rvx}  % steady-state distribution
\newcommand{\td}{W}    % transition distribution
\newcommand{\sdv}{\bp_\rvx}  % steady-state distribution vector
\newcommand{\tdm}{\bW}  % transition distribution matrix
\newcommand{\tde}{w}    % transition distribution matrix elements
\newcommand{\sde}{p}    % steady-state distribution vector elements
\newcommand{\bigO}{\mathcal{O}}



==> macros/gww_theorems.tex <==
% GWW DEFINITIONS AND ABBREVIATIONS
% Edited by Polina Golland -- Jan 14, 2007



\usepackage{amsthm}


\theoremstyle{definition} 
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\theoremstyle{plain}


% THEOREM ENVIRONMENTS


\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corol}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{identity}{Identity}
\newtheorem{defn}{Definition}

\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}

\newtheoremstyle{parant}{}{}{\itshape}{}{\bfseries}{.}{.5em}{#1 \thmnote{(#3)}}
\theoremstyle{parant}
\newtheorem{thmpar}{Theorem}

\theoremstyle{plain}

% \newenvironment{proof}%
% {\noindent{\em Proof: } \begin{singlespace} \small \noindent}%
% {\noindent\qed \end{singlespace}}


\newenvironment{new-proof}[1]%
{ {\em Proof of #1: } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newenvironment{new-new-proof}
{ {\em Proof. } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newtheorem{quest}{Question}


% Defining Starred sections
\newenvironment{starsec}%
{\renewcommand{\thesection}{\arabic{section}*}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}*}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}*}}%
{\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}}}


